Abductive Commonsense Reasoning

Abductive reasoning is inference to the most plausible explanation. For example, if Jenny finds her house in a mess when she returns from work, and remembers that she left a window open, she can hypothesize that a thief broke into her house and caused the mess, as the most plausible explanation. While abduction has long been considered to be at the core of how people interpret and read between the lines in natural language (Hobbs et al., 1988), there has been relatively little research in support of abductive natural language inference and generation. We present the first study that investigates the viability of language-based abductive reasoning. We introduce a challenge dataset, ART, that consists of over 20k commonsense narrative contexts and 200k explanations. Based on this dataset, we conceptualize two new tasks -- (i) Abductive NLI: a multiple-choice question answering task for choosing the more likely explanation, and (ii) Abductive NLG: a conditional generation task for explaining given observations in natural language. On Abductive NLI, the best model achieves 68.9% accuracy, well below human performance of 91.4%. On Abductive NLG, the current best language generators struggle even more, as they lack reasoning capabilities that are trivial for humans. Our analysis leads to new insights into the types of reasoning that deep pre-trained language models fail to perform--despite their strong performance on the related but more narrowly defined task of entailment NLI--pointing to interesting avenues for future research.

==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> sections/bayes.tex <==
\section{Bayesian Modeling for \abnli}
\comment{KS: another way to formulate \abnli, based on a disucussion with Yejin. Feel free to add/remove this section.}

We attempt to formulate \abnli in the context of Bayesian framework.

We define \abnli (note: this is not RTE.) as follows:
\begin{align}
f(M;B,E) &:= f(M;B) + f(M;E) \\ \nonumber
f(M;B) &= \plm(M|B) \\ \nonumber
f(M;E) &= \tilde{p}(M|E) \\ \nonumber
       &= \frac{\plm(E|M)\plm(M)}{\plm(E)}\\ \nonumber
       &\propto  \plm(E|M) \times \plm(M) \nonumber
\label{eq:snli}
\end{align}

Here, $f(y;x)$ is a scoring function which computes a plausibility of $y$ given $x$.
One intuitive way to design $f$ is using probabilities from a language model $p(y|x)$.

==> sections/related_work_orig.tex <==
\section{Background and Related Work}

\citet{peirce1965collected} first defined abduction as the process of forming explanatory hypotheses and characterized it as \textit{``the only logical operation which introduces any new idea"}. 
% \textit{Abduction} was originally introduced by \citet{peirce1965collected} as a form of logical inference of identifying the most plausible explanatory hypothesis for a set of observations. Peirce characterized abduction as ``the only logical operation which introduces any new idea.'' 
Applications of abductive reasoning range from criminal investigation \citep{carson2009abduction} and root-cause analysis \citep{Schoenfisch2015UsingAI} to medical diagnosis \citep{Pople1973OnTM}. % More specifically, in artificial intelligence (AI),
In AI, abductive reasoning has been applied to hypothesis generation in first-order logic systems \citep{morgan1971hypothesis}, case-based reasoning \citep{leake1995abduction, satoh1998using}, vision \citep{charniak1985introduction} and  natural language understanding \citep{Norvig1983FrameAI, wilensky1983planning, hobbs1998syntax, stickel1991prolog, Ng1990OnTR, nagao1989semantic}. 

%While abductive reasoning plays a critical role in humans being able to reasonably fill-in the gaps in a narrative, it has remained understudied in natural language processing (NLP) research. 
While abduction plays a critical role in our abilities to reason about missing elements of a narrative, it remains widely understudied in recent natural language processing (NLP) research. 
Previous work in abductive reasoning has relied on logical representations of thoughts, concepts, and inference rules. The initial barrier of encoding knowledge and text as logical forms is both brittle and hard to scale up in order to cover the rich and complex space of natural language. 
% one that even well funded projects such as Cyc \cite{lenat1990cyc} failed to overcome. <<<--- we don't have evidence they tried to do anything with abduction
In contrast, our work leverages recent advances in neural networks to directly encode natural language. %While we work with the full generality of natural language, we make some simplifying assumptions and formulate \task{} as a binary classification task rather than a hypothesis generation task. 
While we work with the full generality of natural language, we formulate \task{} as a binary classification problem rather than a hypothesis generation task, therefore facilitating easy evaluation of new approaches and encouraging future contributions.

% Need to fit this in somewhere:
% Previously, weighted abduction \cite{hobbs1993interpretation,blythe2011implementing} has moved in this direction. 


% Abduction was first introduced as a concept in the logic of science by \citet{peirce1965collected}, who argued that abduction is a form of logical inference that involves adopting the most explanatory hypothesis for an observation. A wide range of literature \cite{paavola2004abduction, niiniluoto1999defending, flach2013abduction, magnani2011abduction, aliseda2003mathematical} from the philosophy community provides exposition for the use of abductive reasoning as a feasible form of inference.
% \doug{One possible rewrite:  Abduction was first introduced in the philosophy of logic by \citet{peirce1965collected}, who defined abduction as a form of logical inference that involves adopting the most explanatory hypothesis for an observation.  In subsequent years, philosophers have continued to study abduction and distinguish it from other forms of inference, such as deduction and induction \cite{paavola2004abduction, niiniluoto1999defending, flach2013abduction, magnani2011abduction, aliseda2003mathematical}. }

% In artificial intelligence (AI), abductive reasoning has been utilized for hypothesis generation in a first-order logic system \cite{morgan1971hypothesis}, natural language understanding \cite{Norvig1983FrameAI, wilensky1983planning, hobbs1998syntax, stickel1991prolog, Ng1990OnTR, nagao1989semantic}, case-based reasoning \cite{leake1995abduction, satoh1998using} and vision \cite{charniak1985introduction}. More generally, abuctive reasoning has been used in applications such as criminal investigation \cite{carson2009abduction}, root-cause analysis \cite{Schoenfisch2015UsingAI} and medical diagnosis \cite{Pople1973OnTM}. 

% On the other hand, \citet{Josephson2000AbductiveIC} argues the necessity of commonsense reasoning capabilities for systems performing abductive reasoning.

% can be traced to \citet{morgan1971hypothesis}, who utilized abduction for hypothesis generation in a first-order logic system. Subsequently, abduction was suggested as a feasible inference method in several AI applications such as natural language understanding \cite{Norvig1983FrameAI, wilensky1983planning, hobbs1998syntax, stickel1991prolog, Ng1990OnTR, nagao1989semantic}, case-based reasoning \cite{leake1995abduction, satoh1998using}, vision \cite{charniak1985introduction} and others. 
 

% \citet{Josephson2000AbductiveIC} provides a comprehensive overview of the adaptation of abductive reasoning in AI and additionally, argues for the necessity of commonsense reasoning capabilities for systems performing abductive reasoning. 




% While abduction is commonly used in applications such as criminal investigation \cite{carson2009abduction}, root-cause analysis \cite{Schoenfisch2015UsingAI} and medical diagnosis \cite{Pople1973OnTM},
% the earliest incorporation of abductive reasoning in artificial intelligence can be traced to \citet{morgan1971hypothesis}, who utilized abduction for the purpose of hypothesis generation in a first-order logic system. 
%\citet{peng2012abductive, reggia1983diagnostic} offered an alternative formalism for abductive reasoning, using the parsimonious covering theory, where the premise and hypothesis are represented by a causal associative network. 
%\citet{Pople1973OnTM} attempted to use abductive reasoning for medical diagnosis in a theorem proving framework. 


% Those familiar with a few of these works may be getting a clearing picture of why, despite its presence in numerous fields, abduction is not a go-to tool or task in ML; as far as we are aware, work in abductive reasoning has ubiquitously assumed representations of thoughts, concepts, and inference rules. This creates a massive initial barrier of information encoding before meaningful hypotheses can be reasoned about, one that even well funded projects such as Cyc \cite{lenat1990cyc} failed to overcome.  

% \paragraph{Abduction in AI}
% For instance, they illustrate the importance of resolving the local pragmatics of text such as coreference, metonymy and word sense to perform abductive inference. More generally, they emphasize the \textit{commonsensical} nature of abductive inference.

% Our work helps generalize previous work on weighted abduction \cite{hobbs1993interpretation,blythe2011implementing} by significantly scaling up the scope of natural language and also using the expressive power of deep neural networks.


% attempt to cre taeby suggesting that massive models pre-trained on massive data contain strong enough \textit{foundational representations} that they can perform \textit{shallow} abduction that relies on surface forms and, given a richer learning source in which abductive hypotheses are tested, learning deeper \textsc{Neural Abductive Reasoning}.

\paragraph{Entailment vs. Abduction}
The formulation of entailment NLI is closely related to \task{}, but there are two critical distinctions that make abductive reasoning uniquely challenging. First, abduction requires reasoning about commonsense implications of observations (e.g., $H$: ``it rained earlier'' $\implies$ $O$: ``the grass is wet'') which go beyond the linguistic notion of entailment (also noted by \citet{Josephson2000AbductiveIC}).\footnote{$H$ is an explanatory hypothesis and $O$ is an observation.} Second, abduction requires non-monotonic reasoning about a set of commonsense implications collectively, to check the potential contradictions against multiple observations and to compare the level of plausibility of different hypotheses. This makes abductive reasoning distinctly challenging compared to other forms of reasoning such as induction and deduction \citep{shank1998extraordinary}. Perhaps more importantly, abduction is closely related to the kind of reasoning humans perform in everyday situations, where information is incomplete and definite inferences cannot be made. 
% Abduction is special in that it is ampliative -- i.e. it requires exploring hypotheses that go beyond what is logically contained in the \textit{premise}, generating new information from foundational knowledge to justify observations. 

% In previous work, \citet{Josephson2000AbductiveIC} argues for the necessity of commonsense reasoning capabilities for systems performing abductive reasoning. 

\paragraph{Cloze-Style Tasks}

Since abduction is fundamentally concerned with \textit{reasonable} chains of cause-and-effect, our work draws inspiration from previous works that deal with narratives such as script learning \citep{schank1975scripts} and the narrative cloze test \citep{chambers-jurafsky:2009:ACLIJCNLP,jans-EtAl:2012:EACL2012,pichotta-mooney:2014:EACL,rudinger-EtAl:2015:EMNLP}. Rather than learning prototypical scripts or narrative chains, we instead reason about the most plausible events conditioned on observations. We make use of the ROCStories dataset \citep{rocstories}, which was specifically designed for the narrative cloze task. But, instead of reasoning about plausible event sequences, our task requires reasoning about plausible explanations for narrative omissions.

\paragraph{Datasets}

% In spite of being a critical reasoning capability, abductive reasoning has remained an understudied problem. While several datasets aimed at understanding narrative text \cite{rocstories,zellers2018swagaf} and natural language inference \cite{snli:emnlp2015,multinli,copadataset,dagan2006pascal} have been proposed, none of them focus on abductive reasoning.   

Our new resource \dataset{} complements ongoing efforts in building resources for natural language inference \citep{dagan2006pascal,maccartney2009,snli:emnlp2015,multinli,camburu2018snli}. Existing datasets have mostly focused on textual entailment in a deductive reasoning set-up \citep{snli:emnlp2015, multinli} and making inferences about plausible events \citep{copadataset,ordinalci}. In their typical setting, these datasets require a system to \textit{deduce} the logically entailed consequences of a given \textit{premise}. In contrast, the nature of abduction requires the use of commonsense reasoning capabilities, thereby reducing the focus on lexical entailment. While abductive reasoning has been applied to entailment datasets \citet{raina2005robust}, they have been applied in a logical theorem-proving framework as an intermediate step to perform textual entailment -- a fundamentally different task than abductive reasoning. 
% Our task differs from previous work as it requires the use of non-monotonic reasoning by coupling information from two endpoints of a story. 

 

% \citet{camburu2018snli} extend this standard setup by supplementing SNLI \cite{snli:emnlp2015} with natural language explanations and using these explanations for training and providing interpetable justifications. 

% \cscomment{Also include the point about NLI often being lexical distinct from our case. check section 1.3 in intro and reiterate. }

% \cscomment{talk about e-SNLI shortly and describe why this is different?}

% \keisuke{related work section might be better fit before conclusion?, i.e., it sounds better? to dive into the task definition after the intro}
% \keisuke{I add some quotes for reference.}
% \begin{quote}
% \textit{Abduction, or inference to the best explanation}, is a form of inference that goes from data describing something to a hypothesis that best explains or accounts for the data. \cite{Josephson2000AbductiveIC}
% \end{quote}


%There have also been previous efforts to study abductive reasoning… [Other work looking at abductive reasoning (and maybe a brief description of the history of abductive reasoning philosophically - include \cite{raina2005robust}]

%\comment{[hr]
%roughly ordered:\\
%Script Learning and Narrative Cloze (and reltd):
%\begin{itemize}
%\item Script theory - \cite{schank1975scripts}
%\item Narrative Chain - (copied from Keisuke) \cite{chambers-jurafsky:2009:ACLIJCNLP,jans-EtAl:2012:EACL2012,pichotta-mooney:2014:EACL,rudinger-EtAl:2015:EMNLP} - this paper, rather than learning prototypical scripts or narrative chains, is reasoning about what likely events should take place conditioned on instantiated events. 
%\item Roc Story -\cite{rocstories} - this paper uses roc stories to present abductive complement to original dataset, created in a way to avoid stylistic artifacts (avoid saying that too negatively)
%\end{itemize}
%NLI - SNLI datasets\cite{snli:emnlp2015,multinli}, other nli references \cite{dagan2006pascal,maccartney2009} - represent deductive reasoning, this dataset could be complementary, reasoning about what's most plausible rather than factual entailment and also reasoning about multiple points of inference (B$\rightarrow$M and M $\rightarrow$E) \\
%Causal Inference Resources - \cite{copadataset,ordinalci}\\
%Abductive Reasoning -  \cite{raina2005robust}\\
%}


%%% commented out because it is addressed above (thanks!). this will be removed later on.
%\comment{[ks] There is a line of work for script induction,narrative chain, or narrative cloze task.\cite{chambers-jurafsky:2009:ACLIJCNLP,jans-EtAl:2012:EACL2012,pichotta-mooney:2014:EACL,rudinger-EtAl:2015:EMNLP}. We might want to explain the difference.}

% \paragraph{Contrast with current problems and approaches}
% \begin{enumerate}
%     \item Compared to NLI: NLI represents deductive reasoning. So is ROCStories. 
%     \item Cloze test: X
% \end{enumerate}

% \begin{enumerate}
%     \item Scripts
%     \item Narrative cloze test and NLI
%     \item Abductive NLI paper \cite{raina2005robust}: 
% \end{enumerate}

%%%%%%%%%%%%%%%
%%% ATTENTION : Copied text. Rephrase
%%%%%%%%%%%%%%%
% \cite{Xie2017NeuralTG}
%  Perplexity does not always correlate well with downstream metrics \cite{Chen1998EvaluationMF}, automated or otherwise. 
 
%  Common metrics based on n-gram overlap such as ROUGE \cite{lin2004rouge} and BLEU \cite{Papineni2002BleuAM} are only rough approximations, and often do not capture
% linguistic fluency and cohererence \cite{conroy2008mind,Liu2016HowNT}  Such metrics are especially problematic in more open-ended generation tasks such as summarization and dialogue.
% Recent results have shown that though automated metrics are not great at distinguishing between systems once performance passes some baseline, they nonetheless are useful for finding examples where performance is poor, and can also be consistent for evaluating similar systems [Novikova et al., 2017]. Thus, despite issues with current automated evaluation metrics, we assume their use for model development; however, manual human evaluation should be interspersed as well.

%%%%%%%%%%%%%%%
%%% ATTENTION : Copied text. Rephrase
%%%%%%%%%%%%%%%

% \cite{raina2005robust}: The paper proposes converting natural language premise and hypothesis from the PASCAL dataset to a logical form using a syntactic dependency graph and hand written rules to find the heads of all nodes in the parse tree. The logical form of the premise and the hypothesis are unified using a model that computes the cost of making assumptions required to unify a pair of predicates in the premise and hypothesis.

% Q. why can't you skip one of the sentences in story cloze test and treat that as abductive task?


% Moved from intro. Mention in related work for completeness
% -- i.e. computing possible alternatives to events -- which continues to be a challenging open problem. More generally, criminal investigation, scientific research, root-cause analysis \cite{Schoenfisch2015UsingAI} and medical diagnosis \cite{Pople1973OnTM} are applications of abductive reasoning. 
% \cscomment{mention these points about AR applications in paragraph 1 or 2 of related work ?}
